Theoretically-Efficient and Practical Parallel DBSCAN

The DBSCAN method for spatial clustering has received significant attention due to its applicability in a variety of data analysis tasks. There are fast sequential algorithms for DBSCAN in Euclidean space that take $O(n\log n)$ work for two dimensions, sub-quadratic work for three or more dimensions, and can be computed approximately in linear work for any constant number of dimensions. However, existing parallel DBSCAN algorithms require quadratic work in the worst case, making them inefficient for large datasets. This paper bridges the gap between theory and practice of parallel DBSCAN by presenting new parallel algorithms for Euclidean exact DBSCAN and approximate DBSCAN that match the work bounds of their sequential counterparts, and are highly parallel (polylogarithmic depth). We present implementations of our algorithms along with optimizations that improve their practical performance. We perform a comprehensive experimental evaluation of our algorithms on a variety of datasets and parameter settings. Our experiments on a 36-core machine with hyper-threading show that we outperform existing parallel DBSCAN implementations by up to several orders of magnitude, and achieve speedups by up to 33x over the best sequential algorithms.

==> approx.tex <==
\subsection{Approximate DBSCAN} \label{sec:approx-dbscan}

\input{figure-quadtree}

For approximate DBSCAN on any constant number
of dimensions, Gan and Tao~\cite{GanT17} following the high-level
structure of Algorithm~\ref{alg:dbscan-highlevel}---they implement
Line 2 using the grid method, and implement Line 4 with an approximate
range query data structure (essentially a quadtree) for each core cell that returns the number of points within
$\epsilon$ plus any number of points within distance
$(\epsilon,(1+\rho)\epsilon]$ (the \textproc{ClusterCore} procedure on
  Line 4 takes an additional parameter $\rho$). 
  %% Their data structure is a $d$-dimensional quadtree~\cite{har2011geometric},
  %% and it is constructed for each core cell.
  See
  Figure~\ref{fig:quadtree} for an illustration.  A cell of side-length
  $\epsilon/\sqrt{d}$ is recursively divided into $2^d$ sub-cells of the
  same size until either the sub-cell becomes empty or has side-length
  at most $\epsilon\rho/\sqrt{d}$.  This forms a tree where each
  sub-cell is a node and its children are the up to $2^d$ non-empty
  sub-cells that it divides into. Each node of the tree stores the
  number of points contained in its corresponding sub-cell. The tree
  has $l=1+\lceil \log_2 1/\rho\rceil$ levels.  Using a hash table to store the
  tree nodes, the data structure can be constructed in
  $O(nl)$ expected work.  A query to an approximate
  range query data structure takes as input any point $p$, and
  parameters $\epsilon$ and $\rho$, and returns an integer that is
  between the number of points in the $\epsilon$-radius of $p$ and the
  number of points in the $\epsilon(1+\rho)$-radius of $p$. The
  queries start a traversal of the quadtree at the root, and
  recursively searches all children whose bounding box intersects with
  the $\epsilon$-radius of $p$. Once either a leaf node is reached or
  a node's bounding box is completely contained in the
  $\epsilon(1+\rho)$-radius of $p$, the search on that path
  terminates, adding the node's count to the total count. 
Once all
  searches terminate, the total count is returned.  Using a fact
  from~\cite{Arya2000}, Gan and Tao show that the number of nodes
  visited by a query is $O(1+(1/\rho)^{d-1})$. Therefore, for constant
  $\rho$ and $d$, the quadtree data structure can be constructed in
  $O(n)$ expected work and queries can be answered in $O(1)$ expected
  work. To determine connectivity between core cells, for each
  core point $p$ in each core cell $C$, we issue an approximate range
  query to each of its neighboring core cells $C'$ and connect $C$ and
  $C'$ in the cell graph if the range query returns a non-zero count.
The number of queries issued is $O(n)$ so the overall work for Line~4 is $O(n)$.

\begin{algorithm}[!t]
\small
  \caption{Parallel Quadtree Construction}\label{alg:quadtree-construct}
\begin{algorithmic}[1]

\Procedure{ConstructQuadTree}{$\mathcal{P}$, $\mathcal{G}$, $\epsilon$, $\rho$, $d$}

\State $\tau := \epsilon \rho / \sqrt{d}$

%\State $\mathcal{Q} := $\Call{Node}{$\mathcal{P}$, $numChildren = |\mathcal{G}|$}
\ParForEach{$g \in \mathcal{G}$}
\State $l := $ the length of cell $g$
\State $\mathcal{Q}_g :=$
  \Call{ConstructHelper}{$g$, $l/2$, $\tau$}
\EndFor

\EndProcedure

\Procedure{ConstructHelper}{c, $l$, $\tau$}

\If{$l \leq \tau$}\label{alg:quadtree-construct:baseif}
\State \Return \Call{LeafNode}{${c}$}
\Else
\State $\mathcal{Q} := \Call{Node}{{c}, 2^d\,$children}
\State Partition $c$ into $2^d$ sub-cells and use $\Call{ParallelIntSort}{}\!\!\!$ \par  \hskip\algorithmicindent to distribute the points in $c$ to the sub-cells
\ParFor{each non-empty sub-cell $c'$}
\State $\mathcal{Q}.\children[c'] :=\Call{ConstructHelper}{c', l/2, \tau}$
%\par  \hskip\algorithmicindent \Call{ConstructHelper}{$g.\mathcal{P}$, $l/2$, $\tau$}
\EndFor
\EndIf

\State \Return $\mathcal{Q}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\myparagraph{Parallel Approximate DBSCAN} We can
execute all of the approximate range queries in parallel, and each
query already takes $O(1)$ work and depth, giving us $O(n)$ work and
$O(1)$ depth for queries.


We now parallelize the construction of the data structure. The
pseudocode is shown in Algorithm~\ref{alg:quadtree-construct}.  We
construct the data structure for all cells in parallel (Line
3--5). The procedure is recursive, starting at the root node of the
tree which represents all of the points in the cell.  Each node of the tree has
access to the points contained in its sub-cell in a contiguous
subarray that is part of a global array (e.g., by storing a pointer to
the start of its points in the global array as well as the number of
points that it represents).  We sort the points in the subarray based
on which of the $2^d$ sub-cells it belongs to (Line 11). Now the
points belonging to each of the child nodes are contiguous, and we can
recursively construct the up to $2^d$ non-empty child nodes independently in
parallel by passing in the appropriate subarray (Lines 12--13). The
recursion stops  when the
sub-cell has side-length at most $\epsilon\rho/\sqrt{d}$ (Lines 7--8).

The sort on each level can be done in $O(n)$ work and $O(\log n)$
depth using parallel integer sorting~\cite{Vishkin10},
since the keys are integers in a constant range. The number of levels
of the tree is $l=1+\lceil \log_2 1/\rho\rceil$ giving an overall work of
$O(nl)$ and depth of $O(l\log n)$.
Combined with the parallel algorithms from Section~\ref{sec:common},
we have the following theorem.

\begin{theorem}
For constant values of $\minpts$ and $\rho$, our approximate Euclidean
DBSCAN algorithm takes $O(n)$ work and $O(\log n)$ depth with high
probability.
\end{theorem}




%% Theory is straight-forward, and can be obtained by some textbook algorithms proposed in the 80s.
%% Easy to parallelize.

%% \begin{algorithm}
%%   \caption{$\rho$--Approximate DBSCAN}\label{alg:approx-dbscan-highlevel}

%%   \begin{flushleft}
%%   \hspace*{\algorithmicindent} \textbf{Input}: A set $\mathcal{P}$ of data points; $\epsilon$; $minPts$; $\rho$ \\
%%   \hspace*{\algorithmicindent} \textbf{Output}: A list $clusters$ of sets of cluster-identities for each data point
%%   \end{flushleft}

%%   \begin{algorithmic}[1]

%%     %% DBSCAN
%%     \Procedure{DBSCAN}{$\mathcal{P}$, $\epsilon$, $minPts$, $\rho$}
%%     \State $\mathcal{G} :=$ \Call{HyperGrids}{$\mathcal{P}$, $\epsilon$}
%%     \State $coreFlags :=$\Call{MarkCore}{$\mathcal{P}$, $\mathcal{G}$, $\epsilon$, $minPts$}
%%     \State $clusters := \{\emptyset\} \times |\mathcal{P}|$
%%     \State \Call{ClusterCore}{$\mathcal{P}$, $\mathcal{G}$, $coreFlags$, $clusters$, $\epsilon$, $minPts$, $\rho$}
%%     \State \Call{ClusterBorder}{$\mathcal{P}$, $\mathcal{G}$, $coreFlags$, $clusters$, $\epsilon$}
%%     \State \Return $clusters$
%%     \EndProcedure
%%   \end{algorithmic}
%% \end{algorithm}


==> exact.tex <==
\section{Parallel DBSCAN Algorithms}\label{sec:theory}
\julian{to merge with section \ref{sec:alg}}
\subsection{Exact DBSCAN}
%First describe the various 2D exact algorithms and provide theoretical analysis
\myparagraph{Overview} Our exact DBSCAN algorithms have the same outline, which is given in Algorithm~\ref{alg:dbscan-highlevel}.
Our new algorithms are grid-based, similar to previous DBSCAN algorithms and implementations~\cite{Gunawan13,GanT17}.
However, when plugging in newly designed substeps with good theoretical guarantees and practical performance, our new algorithms can achieve good performance both theoretically and practically.

The first step is to construct a \hypergrid{} that partitions the input points into grids with diagonal length $\epsilon$. %/\sqrt[d]{\epsilon}$.
We then check whether each point is a core point based on the \hypergrid{}.
After that, we generate a graph where vertices are those grid cells with at least one core point, and edges connect pairs of cells that each contains a core point and they are within distance $\epsilon$.
Then we compute the connectivity of this graph, which reflect the clusters of the core points.
The last step assigns non-core points to the associated clusters.

%Then describe the higher-D exact algorithm and provide theoretical analysis.
%The work of exact DBSCAN is subsumed by finding the nearest neighbor 
Theoretically, the biggest challenge in this approach is generating edges in the graph for the \hypergrid{}.  
The bottleneck in this step is given two sets, to check whether there exist two points in different set that are within a given distance ($\epsilon$ in this case).
This is equivalent to the problem of computing bichromatic closest pairs.
The main component in these BCP algorithms is the nearest neighbor search (NNS) of given points (also referred to as the \emph{post office problem} by Knuth~\cite{knuth}).
Efficient solutions for exact NNS rely on Delaunay triangulations (DT) and other data structures built on top of them.
We now discuss the existing and new efficient sequential solutions, and new algorithms to parallelize them.

%% \myparagraph{2d case}
%% In 2d case an efficient BCP algorithm is straight-forward.
%% We can construct the convex hull (the boarder of the DT) of one set (using $O(n \log n)$ work for $n$ points), and apply a binary search \yan{?} for each point in another set.
%% The work for a binary search is bounded by $O(\log n)$.
%% For each specific point, there can only be at most 20 nearby grid cells to check with, so the number of binary searches per point is at most 20.
%% The overall cost of BCP is therefore $O(n\log n)$.

%% Parallelizing this approach is simple. 
%% Existing work (citations) can generate a convex hull of $n$ points using $O(n \log n)$ work and $O(\log n)$ \yan{check} depth.
%% Parallelizing binary search seems hard, but we can apply all searches simultaneously, so the depth is also $O(\log n)$.
%% Overall, ...




%\subsection{Exact 2D--DBSCAN}

%Thoery.

%% \begin{algorithm}
%%   \caption{2-D Grid-DBSCAN DelaunayClusterCore}\label{alg:2d-grid-cluster-core-dt}
%%   \begin{algorithmic}[1]
%%     \Procedure{ClusterCore-Delaunay}{$\mathcal{P}$, $\mathcal{G}$, $coreFlags$, $clusters$, $\epsilon$, $minPts$}
%%     \State $cores := \{p \in \mathcal{P} : coreFlags[p] = 1\}$
%%     \State $\mathcal{T} :=$\Call{ParallelDelaunayTriangulation}{$cores$}
%%     \State $\mathcal{U} :=$ \Call{ParallelUnionFind}{$|\mathcal{P}|$}
%%     \ParForEach {$edge \in \mathcal{T}$}
%%     \State $\mathcal{U}.$\Call{Link}{$edge.p$, $edge.q$}
%%     \EndFor

%%     \ParForEach {$p \in cores$}
%%     \State $clusterId := \mathcal{U}.$\Call{Find}{$p$}
%%     \State $clusters[p].$\Call{Add}{$clusterId$}
%%     \EndFor

%%     \EndProcedure

%%   \end{algorithmic}
%% \end{algorithm}


==> opt.tex <==
\section{Implementation}\label{sec:implementation}
This section describes implementation details and optimizations to improve the practical performance of our algorithms.


\myparagraph{Cell Construction}
For the grid method, we use a parallel hash table based on linear
probing~\cite{ShunB14}.  We use the parallel cache-oblivious sample sort algorithm
from the Problem Based Benchmark Suite (PBBS)~\cite{BFGS12,SBFG} for
the box method.

\myparagraph{Quadtree}
% \label{sec:quadtree}
We implement the quadtree in
Algorithm~\ref{alg:quadtree-construct} with an optimization to reduce
the height of the tree: we additionally set a threshold for the number
of points in the sub-cell on Line~\ref{alg:quadtree-construct:baseif},
below which the node becomes a leaf node. This reduces the height of
the tree but potentially makes leaf nodes correspond to non-empty
sub-cells with side-length greater than $\epsilon\rho/\sqrt{d}$.
Therefore, when reaching such a leaf node on a query, instead of simply returning
the count, we explicitly count the number of points contained in the
$\epsilon(1+\rho)$-radius of the query point.
%% To support this optimization
%% and the exact
%% range counting query, each node will keep track of its points in the global array.
In addition, we avoid unnecessary tree node traversal by ensuring that each
tree node has at least two non-empty children: when
processing a cell, we repeatedly divide the points until they fall
into at least two different sub-cells.  For the parallel integer sort,
we use the parallel radix sort algorithm from PBBS~\cite{BFGS12,SBFG}.

While we use quadtrees in
approximate DBSCAN in Section~\ref{sec:approx-dbscan}, we also
implement a version of the quadtree to answer range queries for exact
DBSCAN, which is used when computing connectivity in the cell
graph.
We note that the exact version only differs from the approximate version
only in that it terminates the search
%during pruning the tree search, and all other details are the same.
%For exact range counting queries, the tree traversal will
%terminate
when a node's bounding box is completely contained in the
$\epsilon$-radius of the query point or when the node is a leaf.
In
the latter case, we need to explicitly count the number of points
contained in the $\epsilon$-radius of the query point.

For both approximate and exact DBSCAN, we also implement a version of
the quadtree that can be used for marking core points (in particular,
the \textproc{RangeCount} procedure in
Algorithm~\ref{alg:mark-core}). Given a point $p$, instead of looping
through all points in a neighboring cell, we use a quadtree query to
determine the number of points within the $\epsilon$-radius of $p$.


%% We implemented the quadtree data structure introduced in Section
%% \ref{sec:approx-dbscan} and Figure \ref{fig:quadtree} with
%% optimizations to answer \textit{both exact and approximate} range
%% counting, which could be used in marking core points (see Algorithm
%% \ref{alg:mark-core}) and computing cell graph (see Section
%% \ref{sec:cell-connect-opt}) for both exact and approximate DBSCAN.

\myparagraph{Cell Graph Construction} %\label{sec:cell-connect-opt}
The main computation of Line~\ref{alg:dbscan-highlevel:clustercore} of
Algorithm~\ref{alg:dbscan-highlevel} is determining whether two core
cells should be connected in the core graph.  For $d\ge 3$, the
theoretically-efficient BCP algorithm is complicated and unlikely to
perform well in practice (there are no implementations of the
algorithm available, even sequentially).  Instead, we implement two alternate methods
for determining the connectivity between cells. The first method is
the naive version of BCP---we quadratically iterate through the core
points of both cells until finding a pair of points with distance at
most $\epsilon$, and connect the two cells if such a pair is
found. As done by Gan and Tao~\cite{GanT17}, we optimize this process by first
filtering out points further than $\epsilon$ from the other cell
beforehand. Due to being able to break out of the loop once a pair of
points within a distance of $\epsilon$ is found, it is not efficient
to simply parallelize across all the point comparisons as this will
lead to a significant amount of wasted work. Instead, we divide the
points in each cell into fixed-sized blocks, and iterate over all
pairs of blocks. For each pair of blocks, we compute the distances of
all pairs of points between the two blocks in parallel by writing
their distances into an array.  We then take the minimum distance in
the array using a prefix sum, and return if the minimum is at most
$\epsilon$. This approach reduces the wasted work over the naive
parallelization, while still providing ample parallelism within each
pair of blocks. In addition to the parallelism within a BCP call, all BCP calls can run in parallel.
%% and break out early if a pair within a distance of $\epsilon$ is found.
%% For each pair we compute pairwise point distances between the two blocks
%% in parallel and write them into an array; then we perform a parallel
%% reduction with a $min$ operator to obtain the closest point pair
%% distance.
The second method uses the quadtree data structure described earlier. We loop over each point $p$ in one cell,
and query the quadtree of the other cell to check if any points are in
the $\epsilon$-radius of $p$, and if so connect the two cells and
return. All connectivity queries can run in parallel.
For both methods, we only check connectivity between two cells once by having the cell with higher ID responsible for checking connectivity with the cell with lower ID.

%% which
%%  returns the number of points shared between
%% a cell and an $\epsilon$ sphere of a point; we could loop through the
%% points in one cell and for each point, make an query on the other
%% cell, until the range counting returns a value $>0$.  The range
%% counting query can be supported by the quadtree introduced in section
%% \ref{sec:quadtree}.

Finally, we need to find the connected components of the cell graph.
Instead of directly calling a connected components algorithm on the
cell graph after it is fully constructed, we use a parallel lock-free union-find
data structure to maintain the connected components on-the-fly.  This
optimization can reduce calls for checking connectivity between two
cells, as they could already be connected.  For example, assume that
cells $a$, $b$ and $c$ belong to the same component.  After
connecting $a$ with $b$ and $b$ with $c$, we can avoid the
connectivity check between $a$ and $c$ by checking their respective
components in the union-find structure beforehand.  This optimization
was used by Gan and Tao~\cite{GanT17} in the sequential setting, and we extend it to the parallel setting.

%% Since we used a union-find data structure to dynamically prune
%% connectivity checks, there exists an optimal ordering of connectivity
%% checks that maximizes the pruning.

When constructing the cell graph and checking connectivity, we use a heuristic to prioritize the cells based on the number of core points in the cells, and start from the cells with more points.
This is because cells with more points are more likely to have higher connectivity, hence connecting the nearby cells together and pruning their connectivity queries.
%% Once the nearby cells are connected, they do not need to
%% search out for all their neighbors, leading to less computation.
%resulting in more pruning of
%later connectivity queries.
%In the implementation, each cell will issue connectivity queries to
%its neighboring cells.  To increase the effect of pruning, we applied
%a heuristic of ordering the cells that issue the connectivity queries
%by decreasing order of their size since cells with more points are
%more likely to have high connectivity, resulting in more pruning of
%later connectivity queries.
%% The intuition is that the probability of
%% connecting two cells is proportional to the number of points in them, and early connectivity
%% potentially results in more pruning.
This optimization can be less efficient in parallel, since
a connectivity query could be executed before the corresponding query
that would have pruned it in the sequential execution.
To overcome this, we group the
cells into batches, and process each batch in parallel before moving
to the next batch. We refer to this approach as \defn{bucketing}, and
show experimental results for it in Section~\ref{sec:exp}.
To the best of our knowledge, this is optimization is new.
%% In parallel, this could be done by processing cells in batches,
%% which we call bucketing. Experimental results in show that the
%% bucketing has a positive impact on the scalability in some cases.

%% \footnote{We did not implement a
%%   Voronoi diagram version since practical parallel Voronoi diagram
%%   algorithms are based on first generating the Delaunay triangulation,
%%   and so the Delaunay triangulation-based parallel DBSCAN algorithm is
%%   more efficient.}
For 2D cell graph construction, we implemented three versions: one
using Delaunay triangulation,\footnote{In practice, Delaunay triangulation is faster than Voronoi diagram construction in parallel.} one using USEC with line separation, and one using
the BCP implementation described above, but for $d=2$.  The parallel
Delaunay triangulation code is from PBBS~\cite{BFGS12,SBFG}.
%% and is
%% based on the algorithm by Blelloch et al.\,\cite{BGSS2016}.
Our USEC
with line separation implementation uses parallel sample sort to sort
the points by both coordinates, and then serially constructs the
wavefront for each cell, but parallelizes across different cells since
we found that there was enough coarse-grained parallelism across
cells. Only the top and left wavefronts need to be pre-computed for each cell, as this enables all queries to be answered.
The individual queries are also serial, but all queries can be
executed in parallel.



%% Line~\ref{alg:dbscan-highlevel:clustercore} of Algorithm~\ref{alg:dbscan-highlevel}
%% can be computed using a connected component on the cells. To determine whether
%% an edge should be added between two cells in higher-dimensional space, theoretically we
%% should solve the BCP problem, which is too complicated to work well in practice.
%% We implemented two alternative methods for determining the connectivity
%% between two cells. The first method is the naive version of BCP---quadratically
%% iterate through the core
%% points of both arrays until finding a pair with distance $\le\epsilon$; this could
%% be optimized by first filtering out points further than $\epsilon$ from the other
%% grid before the quadratic looping.
%% We parallelize the quadratic looping by dividing the point candidates in each cell
%% into fix-sized blocks, and check the connectivity of the blocks in a quadratic manner
%% and exit early when connectivity is confirmed. The checking of connectivity between two blocks is
%% done in parallel: we compute pair-wise point distances between the two blocks in parallel
%% and write them into an array; then we perform a parallel reduction with a $min$ operator
%% to obtain the closest point pair distance.
%% The second method to check cell connectivity relies on a range counting
%% query that returns the number of points shared between a cell and an $\epsilon$-sphere
%% of a point; we could loop through the points in one cell and for each point,
%% make an query on the other cell, until the range counting returns a value $>0$.
%% The range counting query can be supported by the quadtree introduced in section
%% \ref{sec:quadtree}.

%% Instead of calling a connected component algorithm on the cells, we use a parallel
%% union-find data structure to keep the connected-components on-the-fly as a practical
%% optimization.  This idea was first mentioned in~\cite{GanT17}. Union-find could dynamically
%% prune down excessive cell connectivity calls between pairs that are already connected.
%% For example, assuming cell $a$, $b$ and $c$ should belong to the same cluster, after
%% connecting $a$ with $b$ and $b$ with $c$, we could prune down the connectivity checking
%% between $a$ and $c$ by checking their respective clusters beforehand.

%% Since we used a union-find data structure to dynamically prune down future core-connect
%% calls, there exists an optimal ordering of adding the connecting edges that maximizes the pruning.
%% Since each cell will issue connectivity queries to its neighbor cells,
%% we applied a heuristic of ordering the cells that issue the query by descending number of
%% points inside the cell. The intuition is that the probability of
%% connecting two cells is proportional to the number of points in them, and early connectivity
%% potentially results in more pruning. In parallel, this could be done by processing cells in batches,
%% which we call bucketing. Experimental results in Section~\ref{sec:exp} show that the
%% bucketing has a positive impact on the scalability in some cases.

%% In 2-dimensional cell graph construction, the practical parallel Voronoi diagram
%% algorithms are based on first generating the Delaunay triangulation,
%% so the Delaunay triangulation-based parallel DBSCAN algorithm is more
%% efficient.  We implemented a 2D DBSCAN algorithm using the parallel
%% Delaunay triangulation code from the Problem Based Benchmark
%% Suite~\cite{BFGS12,SBFG} based on a simpler work-efficient algorithm
%% with polylogarithmic depth~\cite{BGSS2016}.

\myparagraph{Cell Neighbor-Finding}
In the algorithms for marking core points, constructing the cell
graph, and marking border points, we need a subroutine to return a
list of non-empty neighboring cells of a cell. The number of possible
neighbors of a cell grows exponentially with the dimension, and so
enumerating of all possible neighboring cells can be inefficient in
practice for high dimensions (although still constant work in theory).
Instead, we insert all the cells in a $k$-d tree~\cite{Bentley1975} (which does binary splitting instead of the $2^d$-ary splitting in quadtrees),
which enables us to perform range queries to obtain just the non-empty
neighboring cells.  The construction of our $k$-d tree is done
recursively, and all recursive calls for children nodes are executed
in parallel. We also sort the points at each level using parallel
sample sort.  Since queries do not modify the $k$-d tree, they can all be
performed in parallel.  In addition, since a cell needs
to find its neighboring cells multiple times throughout the algorithm,
we memoize the result on its first query to avoid repeated
computation.

%% When marking core points, constructing cell graph and marking border points, we
%% need a subroutine to acquire the list of neighbors of a given cell.
%% Since the number of potential neighbors grows exponentially with the dimension, enumerating all possible candidate neighbors is
%% inefficient for higher dimensions.
%% We manage all the cells in a simple $d$-dimensional
%% tree that enable us to perform range queries and obtain the cell neighbors.
%% The construction of the k-d tree is done recursively, and can be
%% performed in parallel by spawning a new thread for the construction call for each child.
%% Since we do not modify the k-d tree during queries, all queries can be performed embarassingly parallel.
%% In addition, we query to find the neighbors of a cell in a lazy manner, and cache the list to avoid
%% repeated computation.


% granularity control of parallel loops?

%% \subsection{Cell Construction} \label{sec:impl:grid-con}

%% \yiqiu{maybe we can replace cell construction description and pseudocode with something simpler}
%% Given a set of points $P$, we impose a hypergrid structure each with diagonal length $\epsilon$ onto the space as shown in algorithm \ref{alg:hyper-grid}. Line \ref{alg:hyper-grid:pair-start} to \ref{alg:hyper-grid:pair-end} builds an array $A$ of cell-id and point-id pairs; a point can be assigned into a cell simply by dividing its coordinates by the cell side length; the cell-ids can be of any type that has a total order. When we perform sample--sort \cite{} on $A$ using a comparator on the cell-ids, after which pairs in $A$ belonging to the same cell will be continguous. Line \ref{alg:hyper-grid:prefix-start} to \ref{alg:hyper-grid:prefix-end} collects the flags indicating the places where the cell transitions occur in $A$, and then perform a parallel prefix-sum \ref{??} on the flags. % todo diagram on parallel prefix sum
%% Line \ref{alg:hyper-grid:compact-start} to \ref{alg:hyper-grid:compact-end} collect the points for each cell, construct the cell data structure and contruct a list $\mathcal{G}$ of length equal to the number of cells, based on offset information in the prefix-summed flags.

%% \begin{algorithm}
%%   \caption{Parallel Hypergrid Construction}\label{alg:hyper-grid}
%%   \begin{algorithmic}[1]
%%     \Procedure{HyperGrids}{$\mathcal{P}$, $\epsilon$}
%%     \State $A = \{pair\} \times |\mathcal{P}|$ \label{alg:hyper-grid:pair-start}
%%     \ParForEach {$p \in \mathcal{P}$}
%%     \State $A[p].first :=$\Call{GridId}{$p$}
%%     \State $A[p].second := p$
%%     \EndFor \label{alg:hyper-grid:pair-end}

%%     \State $A := $\Call{ParallelSampleSort}{$A$}
%%     \State $flags := \{1\} \times |\mathcal{P}|$ \label{alg:hyper-grid:prefix-start}
%%     \ParFor{$(i := 1; i < |\mathcal{P}|; i ++)$}
%%     \If {$A[i].first = A[i-1].first$}
%%     \State $flags[i] := 0$
%%     \EndIf
%%     \EndFor
%%     \State $numGrids := $\Call{ParallelPrefixSum}{$flags$} \label{alg:hyper-grid:prefix-end}

%%     \State $\mathcal{G} := \{\} \times numGrids$ \label{alg:hyper-grid:compact-start}
%%     \State $i := 0$
%%     \ParFor{$(; i < |\mathcal{P}|-1; i ++)$}
%%     \If{$flags[i] \neq flags[i+1]$}
%%     \State $\mathcal{G}[flags[i]] :=$\Call{Grid}{$\mathcal{P}$, $A$, $i$}
%%     \EndIf
%%     \EndFor
%%     \If {$flags[i] \neq numGrids$}
%%     \State $\mathcal{G}[flags[i]] :=$\Call{Grid}{$\mathcal{P}$, $A$, $i$}
%%     \EndIf

%%     \State \Return $\mathcal{G}$ \label{alg:hyper-grid:compact-end}
%%     \EndProcedure
%%   \end{algorithmic}
%% \end{algorithm}


%% \begin{algorithm}
%%   \caption{Parallel ClusterCore}\label{alg:cluster-core}
%%   \begin{algorithmic}[1]
%%     \Procedure{ClusterCore}{$\mathcal{P}$, $\mathcal{G}$, $coreFlags$, $clusters$, $\epsilon$, $minPts$}
%%     \State $\mathcal{U} :=$ \Call{ParallelUnionFind}{$|\mathcal{G}|$}

%%     \ParForEach {$g \in \mathcal{G}$} \label{alg:cluster-core:outerloop} % note, only those containing core points
%%     \ParForEach {$h \in g.$\Call{NeighborGrids}{$\epsilon$}} \label{alg:cluster-core:innerloop} % note, only those containing core points
%%     \If {$\mathcal{U}.$\Call{Find}{$g$} $\neq h$ \textbf{and} $g < h$ \textbf{and} \par
%%      \hskip\algorithmicindent \Call{CoreConnect}{$g$, $h$, $coreFlags$, $\epsilon$}}
%%     \State $\mathcal{U}.$\Call{Link}{$g$, $h$}
%%     \EndIf
%%     \EndFor
%%     \EndFor

%%     \ParForEach {$g \in \mathcal{G}$}
%%     \State $gridCluster := \mathcal{U}.$\Call{Find}{$g$}
%%     \ParForEach {$p \in g.\mathcal{P}$}
%%     \State $clusters[p].$\Call{Add}{$gridCluster$}
%%     \EndFor
%%     \EndFor
%%     \EndProcedure
%%   \end{algorithmic}
%% \end{algorithm}

%% \begin{algorithm}
%%   \caption{CoreConnect}\label{alg:core-connect}
%%   \begin{flushleft}
%%   \hspace*{\algorithmicindent} \textbf{Preliminary: } First filter the points inside each input grid to core-points only, or make this an assumption, i.e. \\
%%   \hspace*{\algorithmicindent} $g1.\mathcal{P} := \{p \in g1.\mathcal{P} : coreFlags[p] = 1\}$
%%   \hspace*{\algorithmicindent} $g2.\mathcal{P} := \{p \in g2.\mathcal{P} : coreFlags[p] = 1\}$
%%   \end{flushleft}

%%   \begin{algorithmic}[1]
%%     \Procedure{CoreConnect-A}{$g1$, $g2$, $\epsilon$}
%%     \ForEach {$p \in g1.\mathcal{P}$}
%%     \If {\Call{RangeCount-QuadTree}{$p$, $\epsilon$, $g2$} > 0}
%%     \State \Return $true$
%%     \EndIf
%%     \EndFor
%%     \State \Return $false$
%%     \EndProcedure

%%     \Procedure{CoreConnect-B}{$g1$, $g2$, $\epsilon$}
%%     \State $g1.\mathcal{P} := \{p \in g1.\mathcal{P} : $\Call{Dist}{$p$,$g2$}$\leq \epsilon\}$
%%     \State $g2.\mathcal{P} := \{p \in g2.\mathcal{P} : $\Call{Dist}{$p$,$g1$}$\leq \epsilon\}$
%%     \ForEach {$p \in g1.\mathcal{P}$}
%%     \ForEach {$q \in g2.\mathcal{P}$}
%%     \If{\Call{Dist}{$p$, $q$}$\leq \epsilon$}
%%     \State \Return $true$
%%     \EndIf
%%     \EndFor
%%     \EndFor
%%     \State \Return $false$
%%     \EndProcedure
%%   \end{algorithmic}
%% \end{algorithm}

%% \subsection{Range Counting}

%% The \textsc{RangeCount} query is used in both algorithm \ref{alg:mark-core} and algorithm \ref{alg:core-connect}. It accepts a hypersphere and a cell, and returns the number of points in their intersection. We provide two implementations for \textsc{RangeCount} as outlined in algorithm \ref{alg:range-count}. \textsc{RangeCount-A} relies on a quadtree which will be explained in section \ref{sec:impl:quadtree}; a simple and practical implementation of \textsc{RangeCount} is also present in algorithm \ref{alg:range-count} as \textsc{RangeCount-B}.

%% \begin{algorithm}
%%   \caption{RangeCount}\label{alg:range-count}
%%   \begin{algorithmic}[1]
%%     \Procedure{RangeCount-A}{$p$, $radius$, $grid$}
%%     \State \Return \Call{RangeCount-QuadTree}{$p$, $radius$, $grid$}
%%     \EndProcedure

%%     \Procedure{RangeCount-B}{$p$, $radius$, $grid$}
%%     \State $flags := \{0\} \times |grid.\mathcal{P}|$
%%     \ParForEach{$q \in grid.\mathcal{P}$} % in reality this is optimized off as a seq-loop
%%     \If{\Call{Dist}{$p$, $q$} $ \leq radius$}
%%     \State $flags[q] := 1$
%%     \EndIf
%%     \EndFor
%%     \State \Return \Call{ParallelSum}{$flags$}
%%     \EndProcedure
%%   \end{algorithmic}
%% \end{algorithm}


%% \begin{algorithm}%\scriptsize
%% \caption{QuadTree-Query}\label{alg:quadtree-query}
%% \begin{algorithmic}[1]

%% \LineComment{input point $p$ with radius, grid $g$ and quadtree $\mathcal{Q}$}
%% \Procedure{RangeCount-QuadTree}{$p$, $radius$, $g$, $\mathcal{Q}$}
%% \State $relation :=$\Call{CircleGrid}{$p$, $radius$, $g$}
%% \If {$relation = include$}
%% \State \Return $|\mathcal{Q}.\mathcal{P}|$
%% \ElsIf {$relation = disjoint$}
%% \State \Return $0$
%% \ElsIf {$relation = intersect$}

%% \If {$\mathcal{Q}.isLeaf$}
%% \State $result := 0$
%% \ForEach{$q \in Q.\mathcal{P}$} % constant loop size
%% \If{\Call{Dist}{$p$,$q$}$\leq radius$}
%% \State $result += 1$
%% \EndIf
%% \EndFor
%% \Else
%% \State $result := 0$
%% \ParForEach{$child \in \mathcal{Q}.children$}
%% \State $result += $\Call{RangeCount-QuadTree}{$p$, $radius$, $g$, $child$}
%% \EndFor
%% \EndIf % is leaf
%% \State \Return $result$
%% \EndIf
%% \EndProcedure

%% \LineComment{in addition to radius $r1$, accepts $\rho$}
%% \Procedure{ApproxRangeCount-QuadTree}{$p$, $r1$, $\rho$, $g$, $\mathcal{Q}$}
%% \State $r2 := r1 \cdot (1 + \rho)$
%% \State $relation1 :=$\Call{CircleGrid}{$p$, $r1$, $g$}
%% \State $relation2 :=$\Call{CircleGrid}{$p$, $r2$, $g$}
%% \If {$relation1 = include$}
%% \LineComment{grid included in inner sphere}
%% \State \Return $|\mathcal{Q}.\mathcal{P}|$
%% \ElsIf {$relation2 = disjoint$}
%% \LineComment{grid disjoint with outer sphere}
%% \State \Return $0$
%% \ElsIf {$relation = intersect$}

%% \If {$\mathcal{Q}.isLeaf$}
%% \State $result := 0$
%% \ForEach{$q \in Q.\mathcal{P}$} % constant loop size
%% \If{\Call{Dist}{$p$,$q$}$\leq r2$}
%% \State $result += 1$
%% \EndIf
%% \EndFor
%% \Else
%% \State $result := 0$
%% \ParForEach{$child \in \mathcal{Q}.children$}
%% \State $result += $\Call{ApproxRangeCount-QuadTree}{$p$, $r1$, $\rho$, $g$, $child$}
%% \EndFor
%% \EndIf % is leaf
%% \State \Return $result$
%% \EndIf

%% \EndProcedure
%% \end{algorithmic}
%% \end{algorithm}

